Cross-Domain Ensemble Distillation for Domain Generalization

Domain generalization is the task of learning models that generalize to unseen target domains. We propose a simple yet effective method for domain generalization, named cross-domain ensemble distillation (XDED), that learns domain-invariant features while encouraging the model to converge to flat minima, which recently turned out to be a sufficient condition for domain generalization. To this end, our method generates an ensemble of the output logits from training data with the same label but from different domains and then penalizes each output for the mismatch with the ensemble. Also, we present a de-stylization technique that standardizes features to encourage the model to produce style-consistent predictions even in an arbitrary target domain. Our method greatly improves generalization capability in public benchmarks for cross-domain image classification, cross-dataset person re-ID, and cross-dataset semantic segmentation. Moreover, we show that models learned by our method are robust against adversarial attacks and image corruptions.

==> supple/_1_introduction.tex <==
This supplementary material presents additional experimental results, further analyses, and implementation details, all of which are omitted from the main paper due to the space limit.

% the typo correction in our main paper, additional analysis results of the proposed components and other experimental materials, all of which are omitted from the main paper due to the space limit. First, Sec.~\ref{sec:supple_xded} and Sec.~\ref{sec:supple_unistyle} present additional analysis results of XDED and UniStyle, respectively. Lastly, Sec.~\ref{sec:supple_other_materials} includes implementation details.

%First, Sec.~\ref{sec:supple_type_correction} corrects our typo in the main paper to avoid misunderstanding. Sec.~\ref{sec:supple_xded} and Sec.~\ref{sec:supple_unistyle} present additional analysis results of XDED and UniStyle, respectively. Sec.~\ref{sec:supple_other_materials} includes implementation details and and instructions for our source code.

% Finally, we attach the partial source codes implemented using Pytorch. The full implementation will be released on publication. 

==> supple/_2_paper_correction.tex <==
\section{Typo correction for Table.9 of our main paper}
\label{sec:supple_type_correction}
Before diving into additional results of our paper, we sincerely apologize for our typo in table 9 of our main paper. Even though we adopted the 40-2 Wide ResNet~\cite{zagoruyko2016wide} as the backbone network for the results of table 9 in our main paper, we wrote it wrong as WRN-28-10. Again, we are respectfully sorry for the typo, and remark that the experiment of table 9 in our main paper is conducted using the same backbone architecture (\ie, WRN-40-2) for a fair comparison, exactly following the protocol~\cite{hendrycks2019benchmarking,hendrycks2019augmix} to measure generalization to unseen corruptions.

%we exactly follow the protocol to measure generalization to unseen corruptions using \emph{the same backbone architecture} for a fair comparison, which is provided by \cite{hendrycks2019benchmarking}.


==> supple/_3_xded.tex <==
\section{Additional analysis results on XDED}
\label{sec:supple_xded}
In this section, we provide in-depth comparative analysis results between XDED and existing flat minima-promoting methods, qualitative/quantitative analysis results delving into the effect of using the ensemble, and additional ablation studies related to XDED. Lastly, we provide additional empirical results on the flatness of local minima (Fig.~\ref{fig:supple_weight_perturbation}).

% to-do:
% \subsection{on How XDED promotes flat minima.}
% \subsubsection{XDED induces high entropy indeed.}
% \subsection{Ensembles matter for generalization ability.}

% high-entropy, 
% Ensemble matters: qualitative (from CSKD), comparison XDED with (DWED, CSKD), maybe? standard benchmarks (cifar-10, cifar-100, imagenet)

% Comparison to flat minima methods (e.g., A-distance, t-sne, overhead against SAM)

% number of classes in a batch

% standard benchmarks (cifar-10, cifar-100, imagenet)
% learning acceleration
% comparison to ensemble methods
% hyperparam-ablation
% input deformation results
% implementation details

% done: implementation details, input deformation results, hyperparam-ablation, comparison to ensemble methods, learning acceleration, standard benchmarks (cifar-10, cifar-100, imagenet)


%\subsection{The Perspective of Flat Minima}
\subsection{Comparison to existing flat minima-promoting methods}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{supple/supple_figure/supple_a_dist_2.pdf}
    \caption{
    Comparison to existing flat minima-promoting methods. Each model is trained on source domains (\ie, Art Painting, Sketch and Photo of PACS) and evaluated on the target domain (\ie, Cartoon of PACS). \textbf{Left}: The divergence ($\mathcal{A}$-distance) between the source domains and the target domain, \textbf{Right}: Generalization performance on the target domain.
    }
    \label{fig:supple_a_dist}
\end{figure*}

%\subsubsection{XDED learns domain-invariant features as well.}
\subsubsection{Domain-invariant feature learning.}
According to Theorem 1 in our main paper, the test loss on the target domain is bounded by three terms: (1) the robust empirical loss, (2) the domain discrepancy between multiple domains, and (3) confidence bound. While our main paper primarily focuses on the empirical evidences verifying that XDED can effectively reduce the first term (\ie, elevate the flatness of local minima where the model converges), this section highlights that XDED also can reduce the second term (\ie, domain discrepancy) as well as the first term. Therefore, we compare XDED with existing flat minima-promoting methods which are dedicated to reducing the first term only. To investigate the effectiveness of XDED in reducing the domain discrepancy, we measure $\mathcal{A}$-distance~\cite{ben2010theory,kifer2004detecting}, following the protocol stated in our main paper. As shown in Fig.~\ref{fig:supple_a_dist} (Left), although existing flat minima-promoting methods can reduce the robust empirical loss term, they fail to reduce domain discrepancy compared to the vanilla method. In contrast, XDED clearly demonstrates its efficacy to lower the distance between source domains and the target domain. This result demonstrates that XDED learns domain-invariant features by enforcing predictive distribution-level consistency between the data with the same label but from different domains, similar to previous approaches to aligning the feature-level distributions of multiple domains. Next, our investigation also reveals that the result of Fig.~\ref{fig:supple_a_dist} (Left) is exactly reflected in the generalization ability of each method. In detail, as shown in Fig.~\ref{fig:supple_a_dist} (Right), XDED clearly outperforms all the flat minima-promoting methods since only it can learn domain-invariant features unlike them, and this difference leads to significant generalization ability as a result. In addition, when equipped with our UniStyle proposed to reduce the domain gap with the target domain, our framework further reduces the domain discrepancy and enhances the generalization ability. With the above results, we argue that both promoting flat minima and learning domain-invariant features are important for better domain generalization ability, and XDED simultaneously achieves these two goals.

% The result of Fig.~\ref{fig:supple_a_dist} (Left) is exactly reflected to the generalization results of each method, which is shown in Fig.~\ref{fig:supple_a_dist} (Right).

% As shown in Fig.~\ref{fig:supple_a_dist} (Right), by promoting flat minima, all the methods including XDED clearly outperform the vanilla method. However, since XDED can learn domain-invariant features, it shows superiority over other baseline methods.

% With the above results, we argue that both planar minima facilitation and domain invariant feature learning are necessary for better domain generalization, and that XDED achieves these two goals simultaneously.

% not only promote flat minima but also learn domain-invariant features for better domain generalization and XDED achieves these two goals at the same time.

% This result supports our view that XDED leads to better generalization ability by not only promoting flat minima but also reducing domain discrepancy.

% To sum it up, we demonstrate that XDED is not limited to encouraging the convergence into flat minima but also helps the model learn domain-invariant features by penalizing the mismatch of the predictive distributions between the data with the same label but \emph{from different domains}.

\iffalse
\begin{table}[!t]
    \centering
    \caption{
    Comparison of the entropy values which each method induces. Note that the entropy values are calculated by averaging over all training samples when the marked domain is the target domain and the maximum of entropy increases as the number of classes increases.
    }
    %\fontsize{9}{11}\selectfont
    \begin{tabularx}{0.8 \textwidth}{
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X}
    \hline
    \multicolumn{1}{l|}{Methods} & Vanilla & MixStyle~\cite{zhou2021domain}  & XDED  \\
    \hline
    \multicolumn{1}{l|}{OfficeHome (Clipart)} & 0.25 & 0.35 & \textbf{0.92} \\
    % sec/iter
    \multicolumn{1}{l|}{PACS (Cartoon)} & 0.01 & 0.03 & \textbf{0.38} \\
    \hline
    \end{tabularx}
    \label{tab:supple_comparison_entropy}
\end{table}
\fi

\subsubsection{High entropy induced by XDED.} To investigate whether XDED induces high entropy in practice, we calculate the prediction entropy values of the learned model and compare the results of XDED with those of baseline methods. As shown in Table.~\ref{tab:supple_comparison_entropy}, XDED induces higher entropy than other methods for all cases. Specifically, in the case of OfficeHome, the entropy of XDED is about 4 times larger than that of the vanilla method. In the case of PACS, entropy values of other methods are close to zero, while XDED induces higher entropy. In addition, we argue that XDED induces high entropy meaningfully, not blindly. Namely, compared to the entropy value of uniform distribution, the entropy values from XDED are reasonable. Thanks to the use of the ensemble which encodes the meaningful information, XDED is not encouraged to pursue blindly high entropy. Also, note that MixStyle has shown its effectiveness in domain generalization, but it cannot make a difference compared to the vanilla method in inducing high entropy since it has been proposed from the perspective of the data augmentation rather than entropy regularization like our approach. This also supports our view that XDED can further enhance generalization ability as an entropy regularization approach by helping the model converge to flat minima.
\input{table/comparison_entropy}

\begin{table}[!t]
    \centering
    \caption{
    Generalization results on the target domain (Clipart of OfficeHome) and required overhead during training.
    }
    %\fontsize{9}{11}\selectfont
    \begin{tabularx}{0.7 \textwidth}{
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X}
    \hline
    \multicolumn{1}{l|}{Methods} & Vanilla & SAM~\cite{foret2021sharpness}  & XDED  \\
    \hline
    \multicolumn{1}{l|}{Accuracy (\%) ($\uparrow$)} & 49.4 & \underline{51.9} & \textbf{55.2} \\
    % sec/iter
    \multicolumn{1}{l|}{Time / iter (ms) ($\downarrow$)} & \textbf{32} & 72 & \underline{33} \\
    \hline
    \end{tabularx}
    \label{tab:supple_flat_minima_cost}
\end{table}
\subsubsection{Convergence into flat minima at a low cost.}
Since there are several ways for convergence into flat minima, we believe that the required overhead to achieve that goal should be considered as another criterion of valuation for a practical usage. Therefore, according to this point of view, we compare XDED with SAM~\cite{foret2021sharpness} which has been proposed to optimize loss sharpness more directly. As shown in Table.~\ref{tab:supple_flat_minima_cost}, XDED shows superior robustness on the unseen domain over SAM. Furthermore, XDED requires negligible overhead while SAM requires the training time more than 2 times longer than the vanilla method and XDED. This is because SAM must additionally compute gradient approximation for the loss sharpness to be optimized, which exposes a trade-off between training complexity and the optimization of the loss sharpness. 
% Although XDED has relatively weak methodological link to convergence to flat minima compared to SAM, we propose it based on the inspiring observation~\cite{zhang2018deep,zhang2019your} that entropy regularization approaches empirically have shown their efficacy in the convergence into flat minima and provide the empirical evidences that it helps the model converge to flat minima indeed. 
On the other hand, SAM's performance is inferior to that of XDED, since it directly promotes a flat minima but cannot learn domain-invariant features, unlike our method. To sum it up, we argue that XDED offers more appealing option for domain generalization in the context of both performance improvement and required overhead.

% We remark that SAM demands additional overhead since it must compute gradient approximation for the loss sharpness to be optimized.

%\subsubsection{Additional Comparison to Existing Flat Minima-Promoting Methods.? Comparison to SAM?}
%\subsubsubsection{A-distance}
%\subsubsubsection{t-SNE}
%\subsubsubsection{Overhead}


\subsection{Ensemble matters for generalization ability.}
\label{sec:supple_standard_benchmarks}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.82\textwidth]{supple/supple_figure/supple_qualitative1_sero.pdf}
    \caption{Prediction scores for misclassified samples from the vanilla method (\ie, Cross-entropy). \textbf{Up}: Well-classified results from XDED, \textbf{Down}: Misclassified results from XDED.
    }
    \label{fig:supple_qualitative}
\end{figure}
\subsubsection{Qualitative analysis.}
To examine how XDED affects the predictions of the learned model in detail, we investigate the softmax scores from the model which is trained on the source domains (\ie, Cartoon, Sketch and Photo of PACS) and evaluated on the target domain (\ie, Art Painting). Specifically, for the misclassified samples from the vanilla method, we assess the differences in the softmax scores from the vanilla method and XDED. First, as shown in Fig.~\ref{fig:supple_qualitative} (Up), XDED can lead to accurate predictions on the samples which the vanilla method confidently misclassifies. For the giraffe sample, the model learned with XDED not only predicts the ground truth successfully but also puts relatively high probability on the similar class (\ie, Dog) while lowering the probabilities of the irrelevant classes (\ie, Guitar and House). Similarly, even in its failure cases, XDED encourages the model to predict with consideration of inter-class relations (\ie, increasing scores for similar classes while suppressing those for irrelevant classes) as shown in Fig.~\ref{fig:supple_qualitative} (Down). By exploiting the ensemble incorporating information of multiple domains, XDED encourages the model to consider richer inter-class relations which may be exploited on the target domain and lead to meaningful predictions even in failure cases. Note that UniStyle is excluded from the results discussed above.

\input{table/comparison_iid}
\subsubsection{Comparison to existing self-KD methods.}
To further assess the impact of the ensemble distillation, we also compare XDED with state-of-the-art self-knowledge distillation (self-KD) methods in spite of sharing a similar methodology. Furthermore considering that our approach does not explicitly depend on domain labels, we investigate the impact of XDED on the standard benchmark datasets for the image recognition task, which assume the independent and identically distributed (i.i.d.) condition. As shown in Table~\ref{tab:comparison_iid}, XDED outperforms not only the vanilla method but also other self-KD methods for all datasets. Considering that XDED is not dedicated to the case under the i.i.d. condition whereas other methods are dedicated to the case under the i.i.d. condition, these experimental results support our view that XDED can provide more meaningful supervisory signals thanks to the use of ensemble which encodes the complementary knowledge from the data with the same label.


\subsection{Additional ablation studies.}
\subsubsection{Learning acceleration.}
\label{sec:supple_convergence}
Our framework also enables faster convergence of the learning process. In generalization on PACS, our effectiveness of learning acceleration is demonstrated. As shown in Fig.~\ref{fig:supple_convergence}, our framework reaches highest performance with less epochs (\ie, 24 epochs) compared to both vanilla method (40 epochs) and MixStyle~\cite{zhou2021domain} (39 epochs). Although the vanilla method requires many iterations to address the domain gaps between source domains, our framework accelerates the learning process via promoting flat minima which produce lower errors in not only source domains but also the target domain. Since MixStyle~\cite{zhou2021domain}, as an augmentation method, synthesizes novel styles via mixing statistics at the feature level, it is inherently limited to requiring as many epochs as possible to address many augmented styles for its best performance. Also, in the context of the actual training time in total, compared to MixStyle, we remark that our method significantly reduces the training complexity. In detail, our method increases training time per iteration by 5\% but requires only 60\% of training epochs and achieves about 1.6 times more performance boost averaged over every target domain of the PACS dataset. The results are summarized in Table~\ref{fig:supple_convergence}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\columnwidth]{supple/supple_figure/learning_acceleration.pdf}
    \caption{Multi-source domain generalization accuracy (\%) versus the number of epochs on the unseen target domain, Art Painting of PACS. Note that all models were trained on the rest three domains of PACS (\ie, Cartoon, Sketch, and Photo) and all methods were trained with the same hyperparameter setting (\eg, batch size and learning rate) on a single RTX 2080 GPU.
    }
    \label{fig:supple_convergence}
\end{figure}

\subsubsection{Comparison with other ensemble methods.}
\label{sec:supple_comparison_ensemble}
Lastly, we compare our framework with other domain generalization methods which adopt ensemble techniques. The comparison analysis is summarized in Table~\ref{tab:comparison_ensemble}. We remark that the proposed method does not require any additional module and is also free from domain labels (Note that our method, thus, seamlessly extends to the single-source domain generalization setting, which is discussed in Sec.4.1 of our main paper.). Nevertheless, our method clearly outperforms other methods in the context of generalization ability. In contrast, DAEL~\cite{zhou2021dael} and DSON~\cite{seo2020learning} show inferior results even though they explicitly exploit domain labels and multiple domain-specific modules (\ie, classifiers and BN layers~\cite{Batchnorm}, respectively.). DAEL is the most similar to our method but clearly different in the sense that DAEL exploits the predictions of an expert as supervisory signals for non-experts on the same instance, but our method constructs the ensemble using multiple instances and exploits it as supervision to model itself. In other words, by learning domain-invariant information through the ensemble of meaningful knowledge contained in different domains, better performance could be achieved even with limited resources.

\begin{table}[!t]
    \centering
    \caption{ Performance boosts over training complexity.
    }
    %\fontsize{9}{11}\selectfont
    \begin{tabularx}{0.7\textwidth}{ 
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X} 
    \hline
    %\multicolumn{1}{l|}{\multirow{2}{*}[0mm]{Methods}} & Classification & Person re-ID \\  \cline{2-3}
    \multicolumn{1}{l|}{Methods} & Millisec / iter & Accuracy boost (\%) \\
    \hline
    
    %\multicolumn{1}{l|}{IN~\cite{ulyanov2016instance}} & \checkmark & \checkmark & 74.0\\
    
    \multicolumn{1}{l|}{ResNet-18} & 34 & -\\
    \multicolumn{1}{l|}{MixStyle~\cite{zhou2021domain}} & 35 & 4.2 \\
    \multicolumn{1}{l|}{\ccol Ours} & \ccol 37 & \ccol 6.9\\
    
    \hline
    \end{tabularx}
    \label{tab:supple_convergence}
    % \vspace{-4mm}
\end{table}


\subsubsection{Impact of hyperparameters.}
We empirically investigated the effect of the two hyperparameters of XDED: $\lambda$ and $\tau$. We examine accuracy of multi-source domain generalization on Sketch of the PACS dataset by varying the values of the hyperparameters $\lambda \in \{ 0.5, 1.0, 2.5, 5.0, 10.0 \} $ and $\tau \in \{ 1.0, 2.0, 4.0, 6.0, 8.0 \} $. The results are summarized in Fig.~\ref{fig:supple_hyperparam}. First, the performance boost is the highest when $ \tau $ is increased from 1.0 to 2.0. However, if $\tau$ exceeds 2.0, the performance boost is somewhat reduced. Next, $\lambda$ also affects the performance. The performance boost commonly increases with the value of $\lambda$. However, the degree of boost is also reduced when $\tau$ is 1.0. To sum it up, the accuracy of our method is generally high and stable when $\lambda$ and $\tau$ are greater than 5.0 and 2.0, and we argue that this result supports our view that our framework does not strongly depend on the specific hyperparameter setting.

\input{table/comparison_ensemble}


\begin{figure}[t]
    \centering
    % \includegraphics[width=1.\textwidth]{figure/fig1.pdf}
    \includegraphics[width=0.9\textwidth]{supple/supple_figure/sketch_ablation_hyperparam.pdf}
    \caption{Multi-source domain generalization accuracy (\%) versus hyperparameters $\lambda$ and $\tau$ on Sketch of the PACS dataset.
    }
    \label{fig:supple_hyperparam}
\end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{supple/supple_figure/deformation_sero.pdf}
    \caption{Test accuracy (\%) on target domains with input deformations. All models are trained under the multi-source domain generalization setting.
    }
    \label{fig:supple_deformation}
\end{figure*}

\subsubsection{Robustness to input deformations.}
\label{sec:supple_input_deformations}
To further assess the quality of the robustness to unseen domains, we measure the changes in test accuracy as the domain gap becomes larger. We simulate larger domain gaps by increasing the degree of input deformations. Specifically, we applied multiple augmentations defined in RandAugment~\cite{cubuk2020randaugment} to images of the unseen target domain (\ie, Cartoon of PACS), and gradually increased the number of deformations\footnote{For a fair comparison, we use the same operations for each setting.}. Similar to the result of table 9 in our main paper, Fig.~\ref{fig:supple_deformation} shows that our method outperforms baseline methods against pixel-level deformations on unseen domains.
% Additional results are presented in the supplementary material.

==> supple/_4_unistyle.tex <==
\section{Additional analysis results on UniStyle}
\label{sec:supple_unistyle}

\input{table/ablation_where_to_whiten}
\subsection{Where to apply UniStyle}
% all the quantitative results above are produced with the ResNet~\citep{resnet} as a backbone network and 
We remark that UniStyle can be applied after arbitrary intermediate layers of the backbone (\ie, ResNet~\cite{resnet}) as a plug-and-play module. Therefore, to investigate the impact of where UniStyle is applied, we evaluate the generalization performance in image classification and person re-ID while varying the locations of where the operation is applied. For a baseline, MixStyle~\cite{zhou2021domain} is adopted and compared with our UniStyle since they share the commonality of being applied to multiple intermediate feature maps.
For brevity, let \textsc{res\#} denote the indexes of residual blocks where the specified operation is applied (\eg, \textsc{res12} means the operation is applied after both the first and second residual blocks). As shown in Table.~\ref{tab:ablation_where_to_whiten}, we observe that UniStyle and MixStyle have a similar trend in both tasks. First, since early layers are known to capture low-level features such as texture or edge information, it is pertinent for both UniStyle and MixStyle to be applied after early layers to remove style bias and synthesize novel styles, respectively. However, UniStyle achieves the best performances on both tasks, which indicates the importance of removing and unifying style bias rather than augmenting novel styles. Next, on the contrary, both operations lead critical performance drop when incorporated with the last layer, \textsc{res4}, since late layers are known to address semantic information (\ie, their statistics would be highly correlated with target labels). In detail, MixStyle perturbs the statistics by interpolating those of two different instances that may have different labels, whereas UniStyle normalizes the feature map of all samples regardless of their labels, resulting in a more critical performance drop. Note that XDED is excluded in results of Table.~\ref{tab:ablation_where_to_whiten}.


\subsection{Comparison with other methods}
Even though UniStyle is not the first that addresses feature-level statistics (\ie, style information), we take notice of its appealing trade-off between performance boost and training complexity and compare it with other related methods. The results are summarized in Table~\ref{tab:supple_comparison_unistyle}. First, UniStyle outperforms SagNet~\cite{nam2021reducing} and MixStyle~\cite{zhou2021domain}, all of which are dedicated to domain generalization. This indicates that directly removing and unifying the style bias is more effective for generalization ability than augmenting feature statistics or learning style-agnostic features.
Next, although BIN~\cite{nam2018batch} and SRM~\cite{lee2019srm} adaptively recalibrate feature statistics and achieve state-of-the-art performance in image recognition tasks, they show inferior results on unseen domains. Last but not least, Deep Whitening Transformation (DWT)~\cite{cho2019image} which is the most similar to UniStyle shows the second-best performance. DWT has been proposed to encourage the feature extractor to naturally encode the whitened feature by enforcing consistency regularization between the covariance matrix of the feature and identity matrix. Nevertheless, as a constraint that is too strong, DWT weakens feature discrimination and excessively throws away content information, resulting in performance that lags behind UniStyle.
\input{table/comparison_unistyle}


==> supple/_5_other_experiment_materials.tex <==
\section{Implementation details}
\label{sec:supple_other_materials}
\label{sec:supple_implementation}
For the task of domain generalization in image classification, we train the models using the sgd optimizer with the cosine learning decay~\cite{loshchilov2016sgdr} and initial learning rate of $10^{-3}$. They are learned for 100 epochs. For batch construction, we use the batch size of 64, and sample 16 instances per class for the proposed XDED. For the task of person re-ID, we also train the models using the sgd optimizer with initial learning rate of 0.05.

%\subsection{Source code}
%Our code materials to reproduce XDED are located in \q{code\_xded} of \q{supple\_ECCV22\_Cross\_Domain\_Ensemble\_Distillation.zip}. We hope that \q{README.md} helps understand to execute the submitted script.

==> table/ablation_components2.tex <==
\begin{table}
\centering
\fontsize{9}{11}\selectfont
\begin{tabularx}{0.48 \textwidth}{
   p{0.11\textwidth}>{\centering\arraybackslash}X
   >{\centering\arraybackslash}X
   >{\centering\arraybackslash}X
   >{\centering\arraybackslash}X}
\toprule
%\multicolumn{1}{l}{\multirow{2}{*}[-3.5mm]{Methods}}&
%\multicolumn{1}{c}{PACS} &
%\multicolumn{1}{c}{Office-Home} &
%\multicolumn{1}{c}{Person Re-ID} \\
\multicolumn{1}{l}{\multirow{2}{*}[-3.5mm]{Methods}}&
\multicolumn{2}{c}{Accuracy} &
\multicolumn{1}{c}{mAP} \\


%\cline{2-4}
\cmidrule(l){2-3} \cmidrule(l){4-4}
& \multicolumn{1}{c}{PACS} & \multicolumn{1}{c}{Office-Home} & \multicolumn{1}{c}{M$\rightarrow$D}\\

\midrule
\multicolumn{1}{l}{Ours}  & 86.4 & (66.9) & 27.4 \\
\multicolumn{1}{l}{w/o UniStyle}  & (82.8) & 66.9 & (24.2) \\
\multicolumn{1}{l}{w/o XDED}  & 82.9 & (64.5) & 26.2 \\

\bottomrule
\end{tabularx}
\vspace{-2mm}
\caption{
asdf Ablation study of the each component in our framework. (M: Market1501, D:Duke)
}
\vspace{-2mm}
\end{table}

==> table/comparison_ensemble2.tex <==
\begin{table}%[!t]
    \centering
    \fontsize{9}{11}\selectfont
    \begin{tabularx}{0.48\textwidth}{ 
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X} 
    \hline
    %\multicolumn{1}{l|}{\multirow{2}{*}[0mm]{Methods}} & Classification & Person re-ID \\  \cline{2-3}
    \multicolumn{1}{l|}{Methods} & Extra $\theta$ & Domain ID & Accuracy \\
    \hline
    %\multicolumn{1}{l|}{DE~\cite{lakshminarayanan2017simple}} & \checkmark & \ding{56} & -\\
    \multicolumn{1}{l|}{DAEL~\cite{zhou2021dael}} & \checkmark & \checkmark & 74.7\\
    \multicolumn{1}{l|}{DSON~\cite{seo2020learning}} & \checkmark & \checkmark & 74.0\\
    \multicolumn{1}{l|}{\ccol Ours} & \ccol \ding{56} & \ccol \ding{56} & \ccol 76.9\\

    
    %& Accuracy(\%) & mAP(\%)\\
    %  \multicolumn{1}{l|}{\emph{Source}: PA} &  69.1 & 86.4\\ %\hline
    %&  Accuracy & mAP \\ \hline
    %\multicolumn{1}{l|}{Vanilla} &  70.4 & 88.2\\ 
    %\multicolumn{1}{l|}{+ UniStyle} &  71.5 & 89.0\\
    %\multicolumn{1}{l|}{+ XDED} & 72.1 &  89.6\\
    \hline
    \end{tabularx}
    \vspace{0.1mm}
    \caption{
    % Comparison of source embedding and ablations of our method on the CUB-200-2011 (CUB) and Cars-196 (Cars) datasets.
    Comparison with other ensemble methods which are dedicated to domain generalization. Extra $\theta$ and Domain ID denote whether each method requires additional networks and domain labels are bound to be given, respectively. Accuracy denotes the average accuracy of each method over PACS and Office-Home.
    }
    % \vspace{-4mm}
\end{table}

==> table/comparison_flat_minima.tex <==
\begin{table}[!t]
    \centering
    \caption{
    Comparison to existing flat minima-promoting methods on Clipart of OfficeHome in the leave-one-domain-out setting. Note that UniStyle is not applied to the result of XDED.
    % Domain generalization results on Clipart of OfficeHome.
    }
    \fontsize{7}{9}\selectfont
    \begin{tabularx}{1.0 \textwidth}{
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X
       >{\centering\arraybackslash}X}
    \hline
    \multicolumn{1}{l|}{Methods} & Vanilla & MaxEnt~\cite{pereyra2017regularizing} & DML~\cite{zhang2018deep} & SAM~\cite{foret2021sharpness} & SWA~\cite{izmailov2018averaging} & SWAD~\cite{cha2021swad} & \ccol XDED \\
    \hline
    \multicolumn{1}{l|}{Accuracy (\%)} & 49.4 & 51.7 & 51.8 & 51.9 & 52.3 & \underline{52.9} & \ccol \textbf{55.2} \\
    % sec/iter
    \hline
    \end{tabularx}
    \label{tab:comparison_flat_minima}
    \vspace{-4mm}
\end{table}

==> table/comparison_soft_targets.tex <==
\begin{table}%[!t]
    \centering
    \begin{tabularx}{0.5\textwidth}{ 
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X |
           >{\centering\arraybackslash}X} 
    \hline
    %\multicolumn{1}{l|}{\multirow{2}{*}[0mm]{Methods}} & Classification & Person re-ID \\  \cline{2-3}
    %Methods & Top-1 \downarrow & Top-5 \downarrow & NLL \downarrow & ECE \downarrow \\
    Methods & NLL & OE (\%) & ECE (\%) & TCOM (\%) \\
    \hline
    %\multicolumn{1}{l|}{DE~\cite{lakshminarayanan2017simple}} & \checkmark & \ding{56} & -\\
    \multicolumn{1}{l|}{Cross-Entropy} & 0.92 & 8.0 & 10.43 & 13.89 \\
    \multicolumn{1}{l|}{Label smoothing} & 0.92 & 0.19 & \textbf{1.68} & 17.37 \\
    \multicolumn{1}{l|}{Mixup} & 1.12 & \textbf{0.0} & 11.53 & 17.25 \\
    \multicolumn{1}{l|}{Manifold} & 1.02 & 9.24 & 11.37 & 12.84 \\
    \multicolumn{1}{l|}{Entropy-Maximization} &1.75 & \textbf{0.0} & 37.87 & 15.13 \\
    \multicolumn{1}{l|}{Ours} & \textbf{0.70} & \textbf{0.0} & 15.79 & \textbf{20.95} \\

    \hline
    \end{tabularx}
    \vspace{0.1mm}
    \caption{
    Top-K error, negative log-likelihood (NLL) and expected calibration error (ECE) on Art Painting of PACS.%
    -Home.
    }
    \label{tab:comparison_soft_targets}
    % \vspace{-4mm}
\end{table}

%\caption{Top-K error, negative log-likelihood (NLL) and expected calibration error (ECE) on the Office-Home.}
%\label{tab:comparison_soft_targets}


==> table/component_ablation.tex <==
\begin{table*}[!t]
    \caption{Ablation study on the proposed components.}
    \vspace{-2mm}
    \footnotesize
    \begin{subtable}{.5\linewidth}
      \centering
        \caption{Image classification on PACS}
        \begin{tabular}{l c}
            \hline
            %\backslashbox{Method}{Model} & ReNet-18 & + res1 
            Model & Accuracy (\%) \\
            \hline
            ResNet-18 & 79.5 \\
            + UniStyle & 82.9 \\
            + UniStyle + XDED & 86.4 \\
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{.5\linewidth}
      \centering
        \caption{Person re-ID from Market1501$\rightarrow$Duke}
        \begin{tabular}{ll}
            \hline
            %\backslashbox{Method}{Model} & ReNet-18 & + res1 
            Model & mAP (\%) \\
            \hline
            ResNet-50 & 19.3 \\
            + UniStyle & 24.0 \\
            + UniStyle $\&$ XDED & 27.4 \\
            \hline
        \end{tabular}
    \end{subtable}
    \label{tab:ablation_component}
\end{table*}

==> table/domainbed_criteria1.tex <==
\begin{table*}
    \centering
    %\resizebox{\textwidth}{!}{
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{lcccccccc}
    %\toprule
    \hline
    \textbf{Algorithm}        & \textbf{ColoredMNIST}     & \textbf{RotatedMNIST}     & \textbf{VLCS}             & \textbf{PACS}             & \textbf{OfficeHome}       & \textbf{TerraIncognita}   & \textbf{DomainNet}        & \textbf{Avg}              \\
    %\midrule
    %\midrule
    \hline
    ERM                       & 57.8 $\pm$ 0.2            & 97.8 $\pm$ 0.1            & 77.6 $\pm$ 0.3            & 86.7 $\pm$ 0.3            & 66.4 $\pm$ 0.5            & 53.0 $\pm$ 0.3            & 41.3 $\pm$ 0.1            & 68.7                      \\
    IRM                       & 67.7 $\pm$ 1.2            & 97.5 $\pm$ 0.2            & 76.9 $\pm$ 0.6            & 84.5 $\pm$ 1.1            & 63.0 $\pm$ 2.7            & 50.5 $\pm$ 0.7            & 28.0 $\pm$ 5.1            & 66.9                      \\
    GroupDRO                  & 61.1 $\pm$ 0.9            & 97.9 $\pm$ 0.1            & 77.4 $\pm$ 0.5            & 87.1 $\pm$ 0.1            & 66.2 $\pm$ 0.6            & 52.4 $\pm$ 0.1            & 33.4 $\pm$ 0.3            & 67.9                      \\
    Mixup                     & 58.4 $\pm$ 0.2            & 98.0 $\pm$ 0.1            & 78.1 $\pm$ 0.3            & 86.8 $\pm$ 0.3            & 68.0 $\pm$ 0.2            & 54.4 $\pm$ 0.3            & 39.6 $\pm$ 0.1            & 69.0                      \\
    MLDG                      & 58.2 $\pm$ 0.4            & 97.8 $\pm$ 0.1            & 77.5 $\pm$ 0.1            & 86.8 $\pm$ 0.4            & 66.6 $\pm$ 0.3            & 52.0 $\pm$ 0.1            & 41.6 $\pm$ 0.1            & 68.7                      \\
    CORAL                     & 58.6 $\pm$ 0.5            & 98.0 $\pm$ 0.0            & 77.7 $\pm$ 0.2            & 87.1 $\pm$ 0.5            & 68.4 $\pm$ 0.2            & 52.8 $\pm$ 0.2            & 41.8 $\pm$ 0.1            & 69.2                      \\
    MMD                       & 63.3 $\pm$ 1.3            & 98.0 $\pm$ 0.1            & 77.9 $\pm$ 0.1            & 87.2 $\pm$ 0.1            & 66.2 $\pm$ 0.3            & 52.0 $\pm$ 0.4            & 23.5 $\pm$ 9.4            & 66.9                      \\
    DANN                      & 57.0 $\pm$ 1.0            & 97.9 $\pm$ 0.1            & 79.7 $\pm$ 0.5            & 85.2 $\pm$ 0.2            & 65.3 $\pm$ 0.8            & 50.6 $\pm$ 0.4            & 38.3 $\pm$ 0.1            & 67.7                      \\
    CDANN                     & 59.5 $\pm$ 2.0            & 97.9 $\pm$ 0.0            & 79.9 $\pm$ 0.2            & 85.8 $\pm$ 0.8            & 65.3 $\pm$ 0.5            & 50.8 $\pm$ 0.6            & 38.5 $\pm$ 0.2            & 68.2                      \\
    MTL                       & 57.6 $\pm$ 0.3            & 97.9 $\pm$ 0.1            & 77.7 $\pm$ 0.5            & 86.7 $\pm$ 0.2            & 66.5 $\pm$ 0.4            & 52.2 $\pm$ 0.4            & 40.8 $\pm$ 0.1            & 68.5                      \\
    SagNet                    & 58.2 $\pm$ 0.3            & 97.9 $\pm$ 0.0            & 77.6 $\pm$ 0.1            & 86.4 $\pm$ 0.4            & 67.5 $\pm$ 0.2            & 52.5 $\pm$ 0.4            & 40.8 $\pm$ 0.2            & 68.7                      \\
    ARM                       & 63.2 $\pm$ 0.7            & 98.1 $\pm$ 0.1            & 77.8 $\pm$ 0.3            & 85.8 $\pm$ 0.2            & 64.8 $\pm$ 0.4            & 51.2 $\pm$ 0.5            & 36.0 $\pm$ 0.2            & 68.1                      \\
    VREx                      & 67.0 $\pm$ 1.3            & 97.9 $\pm$ 0.1            & 78.1 $\pm$ 0.2            & 87.2 $\pm$ 0.6            & 65.7 $\pm$ 0.3            & 51.4 $\pm$ 0.5            & 30.1 $\pm$ 3.7            & 68.2                      \\
    RSC                       & 58.5 $\pm$ 0.5            & 97.6 $\pm$ 0.1            & 77.8 $\pm$ 0.6            & 86.2 $\pm$ 0.5            & 66.5 $\pm$ 0.6            & 52.1 $\pm$ 0.2            & 38.9 $\pm$ 0.6            & 68.2                      \\
    %\bottomrule
    \hline
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{
        DomainBed
        }
    \vspace*{-2mm}
\end{table*}

==> table/domainbed_criteria2_2.tex <==
% \begin{table}
%     \centering
%     %\resizebox{\textwidth}{!}{
%     %\adjustbox{max width=\textwidth}
%     \resizebox{\columnwidth}{!}
%     {
%     \begin{tabular}{lccccccc}
%     \hline
%     \multicolumn{8}{c}{Model selection: leave-one-domain-out cross-validation} \\
%     %\toprule
%     \hline
%     {Methods}        & {CMNIST}     & {RMNIST}     & {VLCS}             & {PACS}             & {OfficeHome}       & {TerraIncognita}   &  {Avg.}              \\
% \hline
% %\midrule
% ERM & 36.7 & 97.7 & 77.2 & 83.0 & 65.7 & 41.4 & 66.9 \\
% IRM & 40.3 & 97.0 & 76.3 & 81.5 & 64.3 & 41.2 & 66.7 \\
% GroupDRO & 36.8 & 97.6 & \underline{77.9} & 83.5 & 65.2 & 44.9 & 66.7 \\
% Mixup & 33.4 & \underline{97.8} & 77.7 & 83.2 & 67.0 & \textbf{48.7} & 67.9 \\
% MLDG & 36.7 & 97.6 & 77.2 & 82.9 & 66.1 & 46.2 & 67.7 \\
% CORAL & 39.7 & \underline{97.8} & \textbf{78.7} & 82.6 & \textbf{68.5} & 46.3 & \textbf{68.9} \\
% MMD & 36.8 & \underline{97.8} & 77.3 & 83.2 & 60.2 & 46.5 & 66.9 \\
% DANN & \underline{40.7} & 97.6 & 76.9 & 81.0 & 64.9 & 44.4 & 67.5 \\
% CDANN & 39.1 & 97.5 & 77.5 & 78.8 & 64.3 & 39.9 & 66.1 \\
% MTL & 35.0 & \underline{97.8} & 76.6 & \underline{83.7} & 65.7 & 44.9 & 67.2 \\
% SagNet & 36.5 & 94.0 & 77.5 & 82.3 & \underline{67.6} & \underline{47.2} & 67.5 \\
% ARM & 36.8 & \textbf{98.1} & 76.6 & 81.7 & 64.4 & 42.6 & 66.7 \\
% VREx & 36.9 & 93.6 & 76.7 & 81.3 & 64.9 & 37.3 & 65.1 \\
% RSC & 36.5 & 97.6 & 77.5 & 82.6 & 65.8 & 40.0 & 66.6 \\
% \hline
% \ccol Ours & \ccol \textbf{46.5} & \ccol 97.7 & \ccol 74.8 & \ccol \textbf{83.8} & \ccol 65.0 & \ccol 42.5 & \ccol \underline{68.4} \\

% \hline

%     \end{tabular}
%     }
%     \vspace{-2mm}
%     \caption{
%         Domain generalization accuracy (\%) on DomainBed. The results compare fifteen methods including ours across six domain generalization benchmark datasets. Note that we adopt leave-one-domain-out cross-validation as a model selection criteria.
%         }
%     \vspace*{-2mm}
%     \label{tab:domainbed}
% \end{table}


\begin{table*}
    \centering
    %\resizebox{\textwidth}{!}{
    %\adjustbox{max width=\textwidth}
    % \resizebox{\columnwidth}{!}
    % {
    %\fontsize{8.7}{9.7}\selectfont
    \fontsize{6.7}{7.7}\selectfont
    \begin{tabularx}{1.0\textwidth} {
    >{\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    %>{\centering\arraybackslash}X|
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    }
    \hline
    \multicolumn{16}{c}{Model selection: leave-one-domain-out cross-validation} \\
    \hline
    
    {} & {ERM} & {IRM} & {GroupDRO} & {Mixup} & {MLDG} & {CORAL} & {MMD} & {DANN} & {CDANN} & {MTL} & {SagNet} & {ARM} & {VREx} & {RSC} & \ccol {Ours} & \\
    \hline
    \multicolumn{1}{l}{CMNIST} & 36.7  & 40.3 & 36.8 & 33.4 & 36.7 & 39.7 & 36.8 & \underline{40.7} & 39.1  & 35.0 & 36.5 & 36.8 & 36.9 & 36.5 & \ccol \textbf{46.5} \\
    \hline
    \multicolumn{1}{l}{RMNIST} & 97.7  & 97.0 & 97.6 & \underline{97.8} & 97.6 & \underline{97.8} & \underline{97.8} & 97.6 &  97.5 & \underline{97.8} &  94.0 & \textbf{98.1} & 93.6 & 97.6 & \ccol 97.7 \\
    
    
    
    \iffalse
    %\toprule
    \hline
    {Methods}        & {CMNIST}     & {RMNIST}     & {VLCS}             & {PACS}             & {OfficeHome}       & {TerraIncognita}   &  {Avg.}              \\
\hline
%\midrule
ERM & 36.7 & 97.7 & 77.2 & 83.0 & 65.7 & 41.4 & 66.9 \\
IRM & 40.3 & 97.0 & 76.3 & 81.5 & 64.3 & 41.2 & 66.7 \\
GroupDRO & 36.8 & 97.6 & \underline{77.9} & 83.5 & 65.2 & 44.9 & 66.7 \\
Mixup & 33.4 & \underline{97.8} & 77.7 & 83.2 & 67.0 & \textbf{48.7} & 67.9 \\
MLDG & 36.7 & 97.6 & 77.2 & 82.9 & 66.1 & 46.2 & 67.7 \\
CORAL & 39.7 & \underline{97.8} & \textbf{78.7} & 82.6 & \textbf{68.5} & 46.3 & \textbf{68.9} \\
MMD & 36.8 & \underline{97.8} & 77.3 & 83.2 & 60.2 & 46.5 & 66.9 \\
DANN & \underline{40.7} & 97.6 & 76.9 & 81.0 & 64.9 & 44.4 & 67.5 \\
CDANN & 39.1 & 97.5 & 77.5 & 78.8 & 64.3 & 39.9 & 66.1 \\
MTL & 35.0 & \underline{97.8} & 76.6 & \underline{83.7} & 65.7 & 44.9 & 67.2 \\
SagNet & 36.5 & 94.0 & 77.5 & 82.3 & \underline{67.6} & \underline{47.2} & 67.5 \\
ARM & 36.8 & \textbf{98.1} & 76.6 & 81.7 & 64.4 & 42.6 & 66.7 \\
VREx & 36.9 & 93.6 & 76.7 & 81.3 & 64.9 & 37.3 & 65.1 \\
RSC & 36.5 & 97.6 & 77.5 & 82.6 & 65.8 & 40.0 & 66.6 \\
\hline
\ccol Ours & \ccol \textbf{46.5} & \ccol 97.7 & \ccol 74.8 & \ccol \textbf{83.8} & \ccol 65.0 & \ccol 42.5 & \ccol \underline{68.4} \\

\hline
\fi

    \end{tabularx}
    % }
    \vspace{-2mm}
    \caption{
        Domain generalization accuracy (\%) on DomainBed. The results compare fifteen methods including ours across six domain generalization benchmark datasets. Note that we adopt leave-one-domain-out cross-validation as a model selection criteria.
        }
    \vspace*{-2mm}
\end{table*}

==> table/domainbed_criteria2_iclr.tex <==
\begin{table*}
    \centering
    %\resizebox{\textwidth}{!}{
    \adjustbox{max width=\textwidth}
    {
    \begin{tabular}{lccccccc}
    \hline
    \multicolumn{8}{c}{Model selection: leave-one-domain-out cross-validation} \\
    %\toprule
    \hline
    \textbf{Algorithm}        & \textbf{CMNIST}     & \textbf{RMNIST}     & \textbf{VLCS}             & \textbf{PACS}             & \textbf{OfficeHome}       & \textbf{TerraIncognita}   & \textbf{Avg}              \\
\midrule
ERM & 36.7 & 97.7 & 77.2 & 83.0 & 65.7 & 41.4 & 66.9 \\
IRM & 40.3 & 97.0 & 76.3 & 81.5 & 64.3 & 41.2 & 66.7 \\
GroupDRO & 36.8 & 97.6 & 77.9 & 83.5 & 65.2 & 44.9 & 66.7 \\
Mixup & 33.4 & 97.8 & 77.7 & 83.2 & 67.0 & \textbf{48.7} & 67.9 \\
MLDG & 36.7 & 97.6 & 77.2 & 82.9 & 66.1 & 46.2 & 67.7 \\
CORAL & 39.7 & 97.8 & \textbf{78.7} & 82.6 & \textbf{68.5} & 46.3 & \textbf{68.9} \\
MMD & 36.8 & 97.8 & 77.3 & 83.2 & 60.2 & 46.5 & 66.9 \\
DANN & 40.7 & 97.6 & 76.9 & 81.0 & 64.9 & 44.4 & 67.5 \\
CDANN & 39.1 & 97.5 & 77.5 & 78.8 & 64.3 & 39.9 & 66.1 \\
MTL & 35.0 & 97.8 & 76.6 & 83.7 & 65.7 & 44.9 & 67.2 \\
SagNet & 36.5 & 94.0 & 77.5 & 82.3 & 67.6 & 47.2 & 67.5 \\
ARM & 36.8 & \textbf{98.1} & 76.6 & 81.7 & 64.4 & 42.6 & 66.7 \\
VREx & 36.9 & 93.6 & 76.7 & 81.3 & 64.9 & 37.3 & 65.1 \\
RSC & 36.5 & 97.6 & 77.5 & 82.6 & 65.8 & 40.0 & 66.6 \\
\hline
\ccol Ours & \ccol \textbf{46.5} & \ccol 97.7 & \ccol 74.8 & \ccol \textbf{83.8} & \ccol 65.0 & \ccol 42.5 & \ccol 68.4 \\

\hline

    \end{tabular}
    }
    \vspace{-2mm}
    \caption{
        Domain generalization accuracy (\%) on DomainBed. The results compare fifteen methods including ours across six domain generalization benchamark datasets. Note that we adopt leave-one-domain-out cross-validation as a model selection criteria.
        }
    \vspace*{-2mm}
    \label{tab:domainbed}
\end{table*}

==> table/officeHome.tex <==
%\begin{center}
%\adjustbox{max width=\textwidth}{%
\begin{table}[!t]
    %\vspace{-2mm}
    \fontsize{8}{10}\selectfont
    \centering
    %\adjustbox{max width=\textwidth}{%
        % \footnotesize
        \caption{
        Leave-one-domain-out generalization results on OffceHome.
        }
        %\fontsize{8.5}{10.5}\selectfont
        \begin{tabularx}{0.75\textwidth}{
        >{\arraybackslash}l|
        >{\centering\arraybackslash}X
        >{\centering\arraybackslash}X
        >{\centering\arraybackslash}X
        >{\centering\arraybackslash}X|
        >{\centering\arraybackslash}X}
        %\toprule
        \hline
        {Methods} & {Artistic} & {Clipart} & {Product} & {Real} & {Avg.} \\
        %\midrule
        \hline
        ResNet-18 & 58.9 & 49.4 & 74.3 & 76.2 & 64.7 \\
        MMD-AE~\cite{li2018domain} & 56.5 & 47.3 & 72.1 & 74.8 & 62.7 \\
        %CCSA~\cite{motiian2017unified} & 59.9 & 49.9 & 74.1 & 75.7 & 64.9 \\
        JiGen~\cite{carlucci2019domain} & 53.0 & 47.4 & 71.4 & 72.7 & 61.2 \\
        CrossGrad~\cite{shankar2018generalizing} & 58.4 & 49.4 & 73.9 & 75.8 & 64.4 \\
        % DDAIG~\cite{zhou2020deep} & 59.2 & 52.3 & 74.6 & \underline{76.6} & 65.5 \\
        %Epi-FCR~\cite{li2019episodic} & 82.1 & 77.0 & 93.9 & 73.0 & 81.5 \\
        %MetaReg~\cite{balaji2018metareg} & 83.7 & 77.2 & 95.5 & 70.3 & 81.7 \\
        %EISNet~\cite{wang2020learning} & 81.8 & 76.4 & 95.9 & 74.3 & 82.1 \\
        L2A-OT~\cite{zhou2020learning} & \underline{60.6} & 50.1 & \underline{74.8} & \textbf{77.0} & 65.6 \\
        SagNet~\cite{nam2021reducing} & 60.2 & 45.3 & 70.4 & 73.3 & 62.3 \\
        %SagNet~\cite{nam2021reducing} & 83.5 & 77.6 & 95.4 & 76.3 & 83.2 \\
        %SelfReg~\cite{kim2021selfreg} & 82.3 & 78.4 & 96.2 & 77.4 & 83.6 \\
        MixStyle~\cite{zhou2021domain} & 58.7 & 53.4 & 74.2 & 75.9 & 65.5 \\
        %L2D~\cite{wang2021learning} & 81.4 & 79.5 & 95.5 & 80.5 & 84.2 \\
        FACT~\cite{xu2021fourier} & 60.3 & 54.8 & 74.4 & \underline{76.5} & \underline{66.5} \\
        DSON~\cite{seo2020learning} & 59.3 & 45.7 & 71.8 & 74.6 & 62.9 \\
        %DAEL~\cite{zhou2021dael} & 59.4 & \underline{55.1} & 74.0 & 75.7 & 66.0 \\
        RSC~\cite{huang2020self} & 58.4 & 47.9 & 71.6 & 74.5 & 63.1 \\
        \hline
        %\cite{pandey2021generalization} & 86.3 & 81.2 & 97.1 & 81.7 & 86.6 \\
        \ccol Ours & \ccol \textbf{60.8} & \ccol \textbf{57.1} & \ccol \textbf{75.3} & \ccol \underline{76.5} & \ccol \textbf{67.4} \\
        \hline
        %DeepAll+Mixup & 76.8 & 74.9 & 95.8 & 66.6 & 78.5 \\
        
        %Ours+SoftMixup & 84.8 & 83.7 & 95.8 & 79.6 & 86.0 \\
        %\bottomrule
        \end{tabularx}
    %}
    \label{tab:officeHome}
    %\vspace{-6mm}
\end{table}
%}
%\end{center}

==> table/pacs.tex <==
% %\begin{center}
% %\adjustbox{max width=\textwidth}{%
% \begin{table}%[!t]
%     % \vspace{-2mm}
%     \fontsize{8.3}{9.8}\selectfont
%     \centering
%     %\adjustbox{max width=\textwidth}{%
%         % \footnotesize
%         \begin{tabular}{lccccc}
%         %\toprule
%         \hline
%         \textbf{Methods} & \textbf{Art} & \textbf{Cartoon} & \textbf{Photo} & \textbf{Sketch} & \textbf{Avg.} \\
%         %\midrule
%         \hline
%         DeepAll & 77.0 & 75.9 & 96.0 & 69.2 & 79.5 \\
%         MMD-AE~\cite{li2018domain} & 75.2 & 72.7 & 96.0 & 64.2 & 77.0 \\
%         CCSA~\cite{motiian2017unified} & 80.5 & 76.9 & 93.6 & 66.8 & 79.4 \\
%         JiGen~\cite{carlucci2019domain} & 79.4 & 75.3 & 96.0 & 71.6 & 80.5 \\
%         CrossGrad~\cite{shankar2018generalizing} & 79.8 & 76.8 & 96.0 & 70.2 & 80.7 \\
%         MASF~\cite{dou2019domain} & 80.2 & 77.1 & 94.9 & 71.6 & 81.0 \\
%         Epi-FCR~\cite{li2019episodic} & 82.1 & 77.0 & 93.9 & 73.0 & 81.5 \\
%         MetaReg~\cite{balaji2018metareg} & 83.7 & 77.2 & 95.5 & 70.3 & 81.7 \\
%         EISNet~\cite{wang2020learning} & 81.8 & 76.4 & 95.9 & 74.3 & 82.1 \\
%         L2A-OT~\cite{zhou2020learning} & 83.3 & 78.2 & 96.2 & 73.6 & 82.8 \\
%         SagNet~\cite{nam2021reducing} & 83.5 & 77.6 & 95.4 & 76.3 & 83.2 \\
%         DAEL~\cite{zhou2021dael} & 84.6 & 74.4 & 95.6 & 78.9 & 83.4 \\
%         SelfReg~\cite{kim2021selfreg} & 82.3 & 78.4 & 96.2 & 77.4 & 83.6 \\
%         MixStyle~\cite{zhou2021domain} & 84.1 & 78.8 & 96.1 & 75.9 & 83.7 \\
%         L2D~\cite{wang2021learning} & 81.4 & 79.5 & 95.5 & 80.5 & 84.2 \\
%         FACT~\cite{xu2021fourier} & 85.3 & 78.3 & 95.1 & 79.1 & 84.5 \\
%         DSON~\cite{seo2020learning} & 84.6 & 77.6 & 95.8 & \textbf{82.2} & 85.1 \\
%         RSC~\cite{huang2020self} & 83.4 & 80.3 & 95.9 & 80.8 & 85.1 \\
%         \hline
%         %\cite{pandey2021generalization} & 86.3 & 81.2 & 97.1 & 81.7 & 86.6 \\
%         \ccol Ours & \ccol \textbf{85.6} & \ccol \textbf{84.2} & \ccol \textbf{96.5} & \ccol 79.1 & \ccol \textbf{86.4} \\
%         \hline
%         %DeepAll+Mixup & 76.8 & 74.9 & 95.8 & 66.6 & 78.5 \\
        
%         %Ours+SoftMixup & 84.8 & 83.7 & 95.8 & 79.6 & 86.0 \\
%         %\bottomrule
%         \end{tabular}
%         \caption{
%         Leave-one-domain-out generalization results on PACS.
%         }
%     %}
%     \label{tab:pacs}
% \end{table}
% %}
% %\end{center}

%\begin{center}
%\adjustbox{max width=\textwidth}{%
\begin{table}[!t]
    % \vspace{-2mm}
    % \fontsize{8.3}{9.5}\selectfont
    \centering
    %\adjustbox{max width=\textwidth}{%
        % \footnotesize
        \caption{
        Leave-one-domain-out generalization results on PACS.
        }
        \fontsize{8}{10}\selectfont
        \begin{tabularx}{0.75 \textwidth}{
        >{\centering\arraybackslash}X|        >{\centering\arraybackslash}X
        >{\centering\arraybackslash}X
        >{\centering\arraybackslash}X
        >{\centering\arraybackslash}X|
        >{\centering\arraybackslash}X}
        %\toprule
        \hline
        \multicolumn{1}{l|}{{Methods}} & {Art} & {Cartoon} & {Photo} & {Sketch} & {Avg.} \\
        %\midrule
        \hline
        \multicolumn{1}{l|}{ResNet-18} & 77.0 & 75.9 & 96.0 & 69.2 & 79.5 \\
        \multicolumn{1}{l|}{MMD-AE~\cite{li2018domain}} & 75.2 & 72.7 & 96.0 & 64.2 & 77.0 \\
        %\multicolumn{1}{l|}{CCSA~\cite{motiian2017unified}} & 80.5 & 76.9 & 93.6 & 66.8 & 79.4 \\
        \multicolumn{1}{l|}{JiGen~\cite{carlucci2019domain}} & 79.4 & 75.3 & 96.0 & 71.6 & 80.5 \\
        \multicolumn{1}{l|}{CrossGrad~\cite{shankar2018generalizing}} & 79.8 & 76.8 & 96.0 & 70.2 & 80.7 \\
        \multicolumn{1}{l|}{MASF~\cite{dou2019domain}} & 80.2 & 77.1 & 94.9 & 71.6 & 81.0 \\
        \multicolumn{1}{l|}{Epi-FCR~\cite{li2019episodic}} & 82.1 & 77.0 & 93.9 & 73.0 & 81.5 \\
        %\multicolumn{1}{l|}{MetaReg~\cite{balaji2018metareg}} & 83.7 & 77.2 & 95.5 & 70.3 & 81.7 \\
        \multicolumn{1}{l|}{EISNet~\cite{wang2020learning}} & 81.8 & 76.4 & 95.9 & 74.3 & 82.1 \\
        \multicolumn{1}{l|}{L2A-OT~\cite{zhou2020learning}} & 83.3 & 78.2 & \underline{96.2} & 73.6 & 82.8 \\
        \multicolumn{1}{l|}{SagNet~\cite{nam2021reducing}} & 83.5 & 77.6 & 95.4 & 76.3 & 83.2 \\
        %\multicolumn{1}{l|}{DAEL~\cite{zhou2021dael}} & 84.6 & 74.4 & 95.6 & 78.9 & 83.4 \\
        \multicolumn{1}{l|}{SelfReg~\cite{kim2021selfreg}} & 82.3 & 78.4 & \underline{96.2} & 77.4 & 83.6 \\
        \multicolumn{1}{l|}{MixStyle~\cite{zhou2021domain}} & 84.1 & 78.8 & 96.1 & 75.9 & 83.7 \\
        \multicolumn{1}{l|}{L2D~\cite{wang2021learning}} & 81.4 & 79.5 & 95.5 & 80.5 & 84.2 \\
        \multicolumn{1}{l|}{FACT~\cite{xu2021fourier}} & \underline{85.3} & 78.3 & 95.1 & 79.1 & 84.5 \\
        \multicolumn{1}{l|}{DSON~\cite{seo2020learning}} & 84.6 & 77.6 & 95.8 & \textbf{82.2} & \underline{85.1} \\
        \multicolumn{1}{l|}{RSC~\cite{huang2020self}} & 83.4 & \underline{80.3} & 95.9 & \underline{80.8} & \underline{85.1} \\
        \hline
        %\cite{pandey2021generalization} & 86.3 & 81.2 & 97.1 & 81.7 & 86.6 \\
        \multicolumn{1}{l|}{\ccol Ours} & \ccol \textbf{85.6} & \ccol \textbf{84.2} & \ccol \textbf{96.5} & \ccol 79.1 & \ccol \textbf{86.4} \\
        \hline
        %DeepAll+Mixup & 76.8 & 74.9 & 95.8 & 66.6 & 78.5 \\
        
        %Ours+SoftMixup & 84.8 & 83.7 & 95.8 & 79.6 & 86.0 \\
        %\bottomrule
        \end{tabularx}
    %}
    \label{tab:pacs}
    \vspace{-4mm}
\end{table}
%}
%\end{center}

==> table/universality_all.tex <==
%\begin{center}
%\adjustbox{max width=\textwidth}{%
\begin{table*}[!t]
    \centering
    %\adjustbox{max width=\textwidth}{%
        \footnotesize
        \begin{tabular}{lccccc}
        %\toprule
        \hline
        \textbf{Methods} & \textbf{Art} & \textbf{Cartoon} & \textbf{Photo} & \textbf{Sketch} & \textbf{Average} \\
        %\midrule
        \hline
        JiGen~\cite{carlucci2019domain} & 79.4 & 75.3 & 96.0 & 71.6 & 80.5 \\
        %JiGen~\cite{carlucci2019domain} (ours) & 80.5 & 74.7 & 96.0 & 72.1 & - \\
        Ours + JiGen & 85.3 & 79.2 & 95.9 & 79.2 & 84.9 \\
        %\hline
        %SagNet~\cite{nam2021reducing} & 83.5 & 77.6 & 95.4 & 76.3 & 83.2 \\
        %Ours + SagNet~\cite{nam2021reducing} & - & - & - & - & - \\
        %\hline
        %SelfReg~\cite{kim2021selfreg} & 82.3 & 78.4 & 96.2 & 77.4 & 83.6 \\
        %Ours+SelfReg & - & - & - & - & - \\
        \hline
        %RSC~\cite{huang2020self} & 83.4 & 80.3 & 95.9 & 80.8 & 85.1 \\
        RSC~\cite{huang2020self} (\textit{our imple}) & 82.8 & 77.6 & 95.7 & 78.6 & 83.7 \\
        Ours+RSC & 84.7 & 81.3 & 96.2 & 82.2 & 86.1 \\
        \hline
        \end{tabular}
    %}
    
    \vspace{-2mm}
    \caption{
        Universality of our proposed framework. Generalization accuracy (\%) on PACS
        }
    \vspace*{-2mm}
    \label{tab:universality_all}
\end{table*}
%}
%\end{center}

==> table/universality_whitening.tex <==
%\begin{center}
%\adjustbox{max width=\textwidth}{%
\begin{table*}[!t]
    \caption{
        Universality of the proposed whitening. Generalization accuracy (\%) on PACS
    }
    \vspace{-2mm}
    \centering
    %\adjustbox{max width=\textwidth}{%
        \footnotesize
        \begin{tabular}{lccccc}
        %\toprule
        \hline
        \textbf{Methods} & \textbf{Art} & \textbf{Cartoon} & \textbf{Photo} & \textbf{Sketch} & \textbf{Average} \\
        %\midrule
        \hline
        JiGen~\cite{carlucci2019domain} & 79.4 & 75.3 & 96.0 & 71.6 & 80.5 \\
        %JiGen~\cite{carlucci2019domain} (ours) & 80.5 & 74.7 & 96.0 & 72.1 & - \\
        Whitening (proposed) + JiGen & 81.8 & 78.5 & 95.7 & 76.8 & 83.2 \\
        %\hline
        %SagNet~\cite{nam2021reducing} & 83.5 & 77.6 & 95.4 & 76.3 & 83.2 \\
        %Ours + SagNet~\cite{nam2021reducing} & - & - & - & - & - \\
        \hline
        SelfReg~\cite{kim2021selfreg} & 82.3 & 78.4 & 96.2 & 77.4 & 83.6 \\
        Whitening (proposed) + SelfReg & - & - & - & - & - \\
        \hline
        %RSC~\cite{huang2020self} & 83.4 & 80.3 & 95.9 & 80.8 & 85.1 \\
        
        %\footnote{We remark that the performance of RSC was not reproduced even though we adopt the official code of the authors. Also, note that this irreproduceability was confirmed at other methods such as FACT~\cite{xu2021fourier} and SelfReg\cite{kim2021selfreg}}
        
        RSC~\cite{huang2020self} (\textit{our imple}) & 82.8 & 77.6 & 95.7 & 78.6 & 83.7 \\
        Whitening (proposed) + RSC & 83.5 & 78.8 & 95.0 & 79.6 & 84.2\footnote{asdffdsaasdffdsaasdf} \\
        
        \hline
        \end{tabular}
    %}
    \label{tab:universality_whitening}
\end{table*}
%}
%\end{center}
